Nanopore Base Calling on the Edge

We developed a new base caller DeepNano-coral for nanopore sequencing, which is optimized to run on the Coral Edge Tensor Processing Unit, a small USB-attached hardware accelerator. To achieve this goal, we have designed new versions of two key components used in convolutional neural networks for speech recognition and base calling. In our components, we propose a new way of factorization of a full convolution into smaller operations, which decreases memory access operations, memory access being a bottleneck on this device. DeepNano-coral achieves real-time base calling during sequencing with the accuracy slightly better than the fast mode of the Guppy base caller and is extremely energy efficient, using only 10W of power. Availability: https://github.com/fmfi-compbio/coral-basecaller

==> Makefile <==
.PHONY: all
all: main.pdf

main.pdf: *.tex *.bib figures/*
	pdflatex main.tex
	bibtex main
	pdflatex main.tex

.PHONY: clean
clean:
	rm *.aux *.log *.out *.pdf

.PHONY: download_from_gdoc
download_from_gdoc:
	./utils/gdoc_to_latex.py \
	 --download-figures \
	 --out content.tex \
	 --docid 2PACX-1vRZ49aCQhTKdPKxNzzafj_u3h_7-Px20hHaJBhOVVt40LQTDAT5KHybKwhnNZIh4maxdceaHdgDR-yB

